Operationalizing Machine Learning: An Interview Study

Organizations rely on machine learning engineers (MLEs) to operationalize ML, i.e., deploy and maintain ML pipelines in production. The process of operationalizing ML, or MLOps, consists of a continual loop of (i) data collection and labeling, (ii) experimentation to improve ML performance, (iii) evaluation throughout a multi-staged deployment process, and (iv) monitoring of performance drops in production. When considered together, these responsibilities seem staggering -- how does anyone do MLOps, what are the unaddressed challenges, and what are the implications for tool builders? We conducted semi-structured ethnographic interviews with 18 MLEs working across many applications, including chatbots, autonomous vehicles, and finance. Our interviews expose three variables that govern success for a production ML deployment: Velocity, Validation, and Versioning. We summarize common practices for successful ML experimentation, deployment, and sustaining production performance. Finally, we discuss interviewees' pain points and anti-patterns, with implications for tool design.

==> sections/lifecycle.tex <==
\subsection{Routine Tasks of MLEs}
\label{subsec:routinetasks}

The production ML lifecycle can be roughly segmented into the following components: data collection and labeling, feature engineering, model training, model validation, deployment, monitoring, and response to bugs. Moving between each task can involve saving and loading artifacts, wrangling data between different formats, changing tools or environments (e.g., programming languages), and collaborating with different stakeholders (e.g., data analysts or business operators). We briefly discuss these tasks in turn.

\topic{Data Collection and Labeling} Data collection spans sourcing new data, wrangling data from sources into a centralized repository, defining criteria for data errors, and cleaning data with respect to such definitions. Data labeling can be outsourced (e.g., Scale AI, Amazon Mechanical Turk) or performed in-house with teams of annotators. More detailed descriptions of data collection, analysis, wrangling and labeling activities can be found in related papers~\cite{kandel2011wrangler, kandel, datacleaning}.

\topic{Feature Engineering and Model Experimentation}
In the feature engineering and model experimentation components of the production ML lifecycle, ML engineers typically focus on improving ML performance, measured via metrics such as accuracy or mean-squared-error. Experiments can be feature-driven or model-driven; for example, an engineer can create a new feature or change the model architecture from tree-based to neural network-based. Many of the participants reported an emphasis on "data-centric AI" while trying to improve performance: rather than trying different models, they preferred to try different feature ideas or collect new data, relying on their domain expertise.

\topic{Model Evaluation and Deployment} A model is typically evaluated by computing a metric (e.g., accuracy) over a collection of labeled data points hidden at training time, or a \emph{validation dataset}, to see if its performance is better than what the currently-running production model achieved during its evaluation phase. At some companies, models can directly be deployed to all of production after this offline evaluation step. Deployment involves reviewing the proposed change, possibly staging the change to increasing percentages of the population or A/B testing on live users, and keeping records of any change to production in case of a necessary rollback. Engineers at other organizations reported a multi-stage deployment process---models are deployed in "shadow" mode (i.e., models make predictions on live data, and these predictions are evaluated internally but hidden from users), then increasing fractions of the population of users. Depending on the organization, each stage can last anywhere between a few days and a multiple months. Metrics are collected and evaluated after every stage to justify deployment to the following stage.

\topic{ML Pipeline Monitoring and Response} Monitoring ML pipelines and responding to bugs involve tracking live metrics (via queries or dashboards), slicing and dicing subpopulations to investigate prediction quality, patching the model with non-ML heuristics for known failure modes, and finding in-the-wild failures and adding them to the evaluation set. Monitoring production models, especially in the absence of real-time labels, requires human labor to inspect the correctness of a subset of live predictions by hand and maintain a queue of potential bugs. Data-related bugs were the most commonly reported, including broken pipelines as well as data distribution shift.

\subsection{The MLOps Stack}
\label{sec:mlopsstack}

ML applications depend on pipelines that span multiple heterogeneous stages or components, such as feature generation and model training. We divide the stack of tools used to construct, orchestrate, and execute these pipelines into four layers that build on top of each other: infrastructure, component, pipeline, and run layers. A diagram of the four layers is shown in~\Cref{fig:stackdiagram}, and common tools used in each layer are described in~\Cref{app:toolstack}. 

% Each layer is typically interfaced via \emph{configuration files}, or configs (e.g., YAML list of hyperparameters to launch a grid search during model training). Config-driven development minimizes changes to the actual application code, or code powering any of the layers.

\topic{Infrastructure Layer} All units of logic require resources to run (e.g., compute, memory, and storage), or infrastructure. Common facets of ML infrastructure are computing clusters (via cloud-based tools such as AWS or GCP or on-prem CPU, or GPU servers), container orchestration (via microservice ecosystems like Kubernetes or Docker Swarm), cloud storage (e.g., AWS S3), development environments (e.g., Visual Studio Code, Jupyter notebooks), and logging and observability services (e.g., Datadog). While many of these tools are open-source, ML and infrastructure engineers must glue them (and tools for other layers in the stack) together with custom code, often resulting in "homegrown" infrastructure (P1, P2, P5, P6, P10, P12). Moreover, sometimes open-source tools must be extended to support custom use-cases in organizations. An example of this is supporting the usage of private Github repos in Jupyter notebooks in cloud-based environments; infrastructure engineers might compile a custom kernel that downloads and installs the private repo so that a data scientist doesn't need to manually set credentials and \texttt{pip install} a package in a private repository themselves. The usage of notebooks varies across organizations, as discussed further in Section~\ref{sec:challenges-pain}. Notebooks are typically used to prototype ideas, but in some organizations, production infrastructure can run notebooks with dynamic parameters (e.g., via Papermill). If notebooks run in production, organizations typically log the resulting notebook from each component's run to be available for future debugging.
 
 \topic{Component Layer} Components, or individual steps in a pipeline, are typically written as functions or scripts and wrapped in operators defined by the pipeline layer. Components can be written in any language, and different languages lend themselves to different kinds of static and data flow analyses. \shreya{TODO: expand on this, talk to Rolando} Feature generation components typically use SQL, Spark, Pandas, or some other data manipulation framework. ML training and experiment components are usually written in Python and leverage common libraries like Pandas, PyTorch, HuggingFace, Scikit-learn, XGBoost, Tensorflow, and Numpy. ML prediction serving components might be written in a compiled or faster language, such as C++, to respect production latency requirements. Monitoring components span a larger variety of languages---depending on the infrastructure and existing software stack, different languages are used. For example, if a stack is largely Kubernetes-based, logging components may be written in Go. If dashboards for monitoring live metrics interface with a database management system that stores the logs (e.g., MongoDB), monitoring components may be written in SQL. 

\topic{Pipeline Layer} Pipelines consist of directed acyclic graphs (DAGs), where each node in the DAG is a separate component, such as transforming raw data to a set of features to be read by a model (featurization). Pipelines can either run ad-hoc or on a schedule; ad-hoc pipelines tend to be used more during development, while scheduled pipelines are typically required in production. Popular open-source tools to construct, schedule, and orchestrate pipelines on a cluster of computing and storage resources (i.e., on top of the infrastructure) include DBT, Airflow, Argo, Kubeflow, Dagster, and TensorFlow Extended. Proprietary tools, such as Vertex AI, also perform these tasks.

\topic{Run Layer} An execution of a pipeline or component is a run, and the same pipeline can produce many different runs. ML engineers often directly inspect the results of runs and use tools to manage run-related metadata such as data, models, and code. Data catalogs can include information about tables, features, schemas. Model registries include information about trained models, such as time trained, lists of features, and validation set metrics (e.g., accuracy). Experiment tracking logs include parameter and metric values for each model trained (e.g., depth of a decision tree and training accuracy). Common open-source tools used in the metadata layer are Weights \& Biases, MLFlow, Amundsen, Hive metastores, and AWS Glue.


In the remainder of the paper, we discuss details of how we performed our qualitative study and insights we learned from the interviews.





==> sections/stack.tex <==
\section{The MLOps Stack}

\begin{figure}
    \centering
\tikzset{description/.append style={top color=\col,bottom color=\col},
 description title/.append style={top color=\col,bottom color=\col}}
    \smartdiagramset{
    % module shape=rectangle,
    % module minimum width=4cm,
    description title font = \scriptsize,
    description width=12cm,
    description text width=12cm,
    % descriptive items y sep=1em,
    set color list={run!50, pipeline!50, component!50, infra!50},
    border color=gray!50!black,
    }
    \resizebox{\linewidth}{!}{
    \smartdiagram[descriptive diagram]{{\bf Run, {Manage metadata for a run of a pipeline (e.g., Weights \& Biases, AWS Glue, metric dashboards)}}, {\bf Pipeline, {Stitch components in a DAG to execute ad-hoc or on a predefined schedule (e.g., Airflow)}}, {\bf Component, {Accomplish individual tasks like model training (e.g., Tensorflow, PyTorch, Scikit-learn)}}, {\bf Infrastructure, {Provide resources to execute components or pipelines (e.g., GCP, AWS S3)}}}}
    \caption{Layers of technical tools in the production ML stack. \jmh{current colors obscure text}}
    \label{fig:stackdiagram}
\end{figure}

